Classical multivariate Hermite coordinate interpolation on n-dimensional grids

In this work, we study the Hermite interpolation on $n$-dimensional non-equally spaced, rectilinear grids over a field $\Bbbk $ of characteristic zero, given the values of the function at each point of the grid and the partial derivatives up to a maximum degree. First, we prove the uniqueness of the interpolating polynomial, and we further obtain a compact closed form that uses a single summation, irrespective of the dimensionality, which is algebraically simpler than the only alternative closed form for the $n$-dimensional classical Hermite interpolation [1]. We provide the remainder of the interpolation in integral form; we derive the ideal of the interpolation and express the interpolation remainder using only polynomial divisions, in the case of interpolating a polynomial function. Moreover, we prove the continuity of Hermite polynomials defined on adjacent $n$-dimensional grids, thus establishing spline behavior. Finally, we perform illustrative numerical examples to showcase the applicability and high accuracy of the proposed interpolant, in the simple case of few points, as well as hundreds of points on 3D-grids using a spline-like interpolation, which compares favorably to state-of-the-art spline interpolation methods.

==> idealconn.tex <==
Let us consider the polynomials $f_{i}\in \Bbbk \left[ x_{i}\right], ~i=1,\dots,n,$  $A_{i}$ the sets of their roots in the algebraic closure $\overline{\Bbbk }$
of $\Bbbk $, and $\nu _{i}\left( a\right) $ the multiplicity of $a\in A_{i}$. 
Therefore $f_{i}\left( x_{i}\right) =\prod_{a\in A_{i}}\left( x_{i}-a\right)
^{\nu _{i}\left( a\right) },~i=1,\dots,n$. 
Furthermore, we denote by $I$ the ideal of $\Bbbk \left[ x_{1},\dots,x_{n}\right] $
generated by $f_{1},\dots,f_{n}$, and by $\overline{I}$ the ideal of $%
\overline{\Bbbk }\left[ x_{1},\dots,x_{n}\right] $ generated by $%
f_{1},\dots,f_{n}$. 
 For $g\in \Bbbk \left[ x_{1},\dots,x_{n}\right] $ let us denote by\ $
\widetilde{g}$ the residue class of $g$ in $\Bbbk \left[ x_{1},\dots,x_{n}%
\right] /I$ , and by $\overline{g}\ $the residue class of $g$\ in $\overline{%
\Bbbk }\left[ x_{1},\dots,x_{n}\right] /\overline{I}$ and $J\left( \mathbf{A,}\nu \right) :=\left\{ f\in \overline{\Bbbk }\left[
x_{1},\dots,x_{n}\right] :\,\partial _{\mathbf{a}}^{\mathbf{m}}f=0,~\mathbf{%
a\in A},\; \mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}\right) -%
\mathbf{1}\right] \right\} $. Similarly to Remark \ref{rem8} it can be shown that $
J\left( \mathbf{A,}\nu \right) $ is an ideal of $\overline{\Bbbk }\left[
x_{1},\dots,x_{n}\right] .$

\begin{lem}\label{lem41}
The $\overline{\Bbbk }$-algebra $\overline{\Bbbk }\left[ x_{1},\dots,x_{n}%
\right] /J\left( \mathbf{A,}\nu \right) $ as a $\overline{\Bbbk }-$vector
space is isomorphic to $V\left( \mathbf{A,}\nu \right) $, and 
\begin{equation*}
\dim _{\overline{\Bbbk }}\overline{\Bbbk }\left[ x_{1},\dots,x_{n}\right]
/J\left( \mathbf{A,}\nu \right) =\prod_{i=1}^{n}\sum_{a_{i}\in A_{i}}\nu
_{i}\left( a\right).
\end{equation*}
\end{lem}

\begin{proof}
Let $\phi :\overline{\Bbbk }\left[ x_{1},\dots,x_{n}\right] \rightarrow 
\overline{\Bbbk }\left[ x_{1},\dots,x_{n}\right] /J\left( \mathbf{A,}\nu
\right) $ be the canonical map and $B\left( \mathbf{A,}\nu \right) :=\left\{ \mathbf{x}^{%
\mathbf{k}}:\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}%
}\nu \left( \mathbf{a}\right) \right] \right\}$ a basis of the vector space $V\left( \mathbf{A,}%
\nu \right) $. It is sufficient to show
that $\phi \left( B\left( \mathbf{A,}\nu \right) \right) $ is a basis of $K%
\left[ x_{1},\dots,x_{n}\right] /J\left( \mathbf{A,}\nu \right)$. Starting
from $\sum_{\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}%
}\nu \left( \mathbf{a}\right) \right] }c_{\mathbf{k}}\phi \left( \mathbf{x}^{%
\mathbf{k}}\right) =0$, we have $\sum_{\mathbf{k\in }\left[ \mathbf{0,}-%
\mathbf{1+}\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}\right) \right] }c_{%
\mathbf{k}}$\textbf{$x$}$^{\mathbf{k}}\in J\left( \mathbf{A,}\nu \right) $,
or equivalently $\partial _{\mathbf{a}}^{\mathbf{m}}\sum_{\mathbf{k\in }%
\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}%
\right) \right] }c_{\mathbf{k}}$\textbf{$x$}$^{\mathbf{k}}=0$, so according
to Corollary \ref{cor24} $\sum_{\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}%
\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}\right) \right] }c_{\mathbf{k}}$%
\textbf{$x$}$^{\mathbf{k}}=0$. That is $c_{\mathbf{k}}=0$, $\mathbf{k\in }%
\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}%
\right) \right]$, which means that $\phi \left( \mathbf{x}^{\mathbf{k}}\right),
\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}\sum_{\mathbf{a\in A}}\nu \left( 
\mathbf{a}\right) \right] $ are linearly indepedend. Now we will show that $%
\phi \left( \mathbf{x}^{\mathbf{k}}\right) ,\mathbf{k\in }\left[ \mathbf{0,}-%
\mathbf{1+}\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}\right) \right] $
generate $\Bbbk \left[ x_{1},\dots,x_{n}\right] /J\left( \mathbf{A,}\nu
\right) $: By Theorem \ref{thm1}, for any $g\in \Bbbk \left[ x_{1},\dots,x_{n}\right] 
$ there is exactly one $f=\sum_{\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}%
\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}\right) \right] }c_{\mathbf{k}}$%
\textbf{$x$}$^{\mathbf{k}}\in V\left( \mathbf{A,}\nu \right) $ such that $%
\partial _{\mathbf{a}}^{\mathbf{m}}f=\partial _{\mathbf{a}}^{\mathbf{m}}g,$ $%
\mathbf{a\in A},~\mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}%
\right) -\mathbf{1}\right]$. Consequently, $\phi \left( g\right) =\phi
\left( f\right) $ or 
\begin{equation*}
\phi \left( g\right) =\sum_{\mathbf{k\in }\left[ \mathbf{0,}-\mathbf{1+}%
\sum_{\mathbf{a\in A}}\nu \left( \mathbf{a}\right) \right] }c_{\mathbf{k}%
}\phi \left( \mathbf{x}^{\mathbf{k}}\right) .
\end{equation*}
\end{proof}

\begin{lem}
%If $\left( f_{1},\dots,f_{n}\right) $ is the ideal of $\Bbbk \left[x_{1},\dots,x_{n}\right] $ generated by the polynomials $f_{1}\in \Bbbk \left[x_{1}\right] ,\dots,f_{n}\in \Bbbk \left[ x_{n}\right] $, then 
The quotient
ring $\Bbbk \left[ x_{1},\dots,x_{n}\right] /I$ as a $\Bbbk$-vector space is
isomorphic to $V\left( \mathbf{A,}\nu \right) $, and  
\begin{equation*}
\dim _{\Bbbk }\Bbbk \left[ x_{1},\dots,x_{n}\right] /I=\prod_{i=1}^{n}\deg
f_{i}=\prod_{i=1}^{n}\sum_{a_{i}\in A_{i}}\nu _{i}\left( a\right) .
\end{equation*}
\end{lem}

\begin{proof}
Clearly, it is sufficient to prove that for any polynomial $f\in \Bbbk \left[ x_{1},\dots,x_{n}%
\right] $ there exist unique $c_{\left( k_{1},\dots,k_{n}\right) }\in K,~0\leq
k_{1}<\deg f_{1},\dots,0\leq k_{n}<\deg f_{n}$, such that 
\begin{equation*}
f=\sum_{k_{1}=0}^{\deg f_{1}-1}\dots\sum_{k_{n}=0}^{\deg f_{n}-1}c_{\left(
k_{1},\dots,k_{n}\right) }x_{1}^{k_{1}}\dots x_{n}^{k_{n}}+I.
\end{equation*}%
To this end we will apply the method of induction over $n$. For $n=1$ obviously the claim is valid. Let the claim be valid for $n-1,n>1$%
. From $f\in \Bbbk \left[ x_{1},\dots,x_{n-1}\right] \left[ x_{n}\right] $, by
dividing $f$ $\ $by $f_{n}\left( x_{n}\right) $, we have $f=pf_{n}+q,$ where 
$p,q\in \Bbbk \left[ x_{1},\dots,x_{n}\right] $ are uniquely determined
by $\deg _{n}q<\deg f_{n}$. Therefore 
\begin{equation}\label{taged31}
f=\sum_{i=0}^{-\deg f_{n}-1}q_{i}x_{n}^{i}+\left( f_{n}\right), 
\end{equation}%
where $q_{i}$ are uniquely determined polynomials of $\Bbbk \left[
x_{1},\dots,x_{n-1}\right] $, and $\left( f_{n}\right) $ is the ideal of $%
\Bbbk \left[ x_{1},\dots,x_{n}\right] $ generated by $f_{n}$. Now by induction
the polynomials $q_{i}$ can be written as, 
\begin{equation}\label{taged32}
q_{i}=\sum_{0\leq k_{1}<\deg f_{1}}\dots \sum_{0\leq k_{n-1}<\deg
f_{n-1}}c_{\left( k_{1},\dots,k_{n-1}\right)
}^{i}x_{1}^{k_{1}}\dots x_{n-1}^{k_{n-1}}+\left( f_{1},\dots,f_{n-1}\right) , 
\end{equation}%
where $c_{\left( k_{1},\dots,k_{n-1}\right) }^{i}\in \Bbbk $ are uniquely
determined$.$ Putting (\ref{taged32}) in (\ref{taged31}) we obtain the claim.
\end{proof}

\begin{thm}\label{them43}
The following holds  
$$\overline{I}=J\left( \mathbf{A,}\nu \right) $$
\end{thm}

\begin{proof}
We can write $f_{i}$ as, $f_{i}\left( x_{i}\right) =\prod_{a\in
A_{i}}\left( x_{i}-a\right) ^{\nu _{i}\left( a\right) },~i=1,\dots,n.$ By
Leibniz derivative rule we easily conclude that for each $g\in \overline{%
\Bbbk }\left[ x_{1},\dots,x_{n}\right] $ is valid $\partial _{\mathbf{a}}^{%
\mathbf{m}}\left( gf_{\iota }\right) =0$, for each $\mathbf{a\in A},~\mathbf{%
m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}\right) -\mathbf{1}\right] .$
Therefore $f_{i}\in J\left( \mathbf{A,}\nu \right) ,~i=1,\dots,n.$ That is 
\begin{equation}\label{taged33}
\overline{I}\subseteq J\left( \mathbf{A,}\nu \right) .
\end{equation}%
It is sufficient \ to show $J\left( \mathbf{A,}\nu \right) \subseteq 
\overline{I}$: Let $g$ be any element of $\overline{I}$. By Lemma \ref{lem41} there
is unique polynomial $p\in V\left( \mathbf{A,}\nu \right) $ such that 
\begin{equation} \label{taged34}
g=p+\overline{I}  
\end{equation}%
From (\ref{taged34}) we have that for any $\mathbf{m\in }\left[ \mathbf{%
0,}\nu \left( \mathbf{a}\right) -\mathbf{1}\right] $ and any$~\mathbf{a\in A}
$ 
\begin{equation*}
\partial _{\mathbf{a}}^{\mathbf{m}}g=\partial _{\mathbf{a}}^{\mathbf{m}}p,
\end{equation*}%
which implies $\partial _{\mathbf{a}}^{\mathbf{m}}p=0$. Therefore by
Corollary 2.4 \ is valid $p=0,$ which combined with (\ref{taged34})
gives $g\in \overline{I}.$
\end{proof}

\begin{cor}
The following holds $$I=J\left( \mathbf{A,}\nu \right) \cap \Bbbk \left[ x_{1},\dots,x_{n}\right].$$
%that is $f\in I$ if and only if $\ \partial _{\mathbf{a}}^{\mathbf{m}}f=0$
%for each $\mathbf{a\in A}$ and$~\mathbf{m\in }\left[ \mathbf{0,}\nu \left( \mathbf{a}\right) -\mathbf{1}\right] .$
\end{cor}

\begin{proof}
By Theorem \ref{them43} we immediately get $I\subseteq J\left( \mathbf{A,}\nu \right)
\cap \Bbbk \left[ x_{1},\dots,x_{n}\right] $. Therefore it is sufficient to
prove $J\left( \mathbf{A,}\nu \right) \cap \Bbbk \left[ x_{1},\dots,x_{n}%
\right] \subseteq I:$ \ Let $f$ be any element of $J\left( \mathbf{A,}\nu
\right) \cap \Bbbk \left[ x_{1},\dots,x_{n}\right] .$ Then by Theorem \ref{them43} we have%
\begin{equation}\label{taged36}
f=\sum_{i=1}^{n}f_{i}g_{i},
\end{equation}%
where $g_{i}\in \overline{\Bbbk }\left[ x_{1},\dots,x_{n}\right] .$ Consider
the finite field extension $\Bbbk \subset \Bbbk _{1}$, where $\Bbbk _{1}$ is
the field constructed by adjunction of all coefficients of the polynomials $%
g_{i}.$ Let $r$ be the degree of $\Bbbk \subset \Bbbk _{1}$ and $\rho $ a
primitive element. Then (\ref{taged36}) can be written as 
\begin{equation}\label{taged37}
f=\sum_{j=0}^{r-1}\rho ^{j}\sum_{i=1}^{n}f_{i}g_{ij},  
\end{equation}%
where $g_{ij}\in \Bbbk \left[ x_{1},\dots,x_{n}\right] .$ Finally, since $%
\left\{ 1,\rho ,\dots,\rho ^{n-1}\right\} $ is $\Bbbk -$ linearly indepedent,
one from (\ref{taged37}) has
\begin{equation*}
f=\sum_{i=1}^{n}f_{i}g_{ij}.
\end{equation*}
\end{proof}
In other words $f\in I$, if and only if $I=J\left( \mathbf{A,}\nu \right) \cap \Bbbk \left[ x_{1},\dots,x_{n}\right]$.


==> rema1.tex <==
\begin{rem}
{\rm
Regarding the \textcolor{black}{computational cost} introduced by the calculation of the formula (\ref{mainform}): Let $n$ be the number of dimensions. Consider the grid $\mathbf{A}=A_1 \times \dots \times A_n$, and $N_1=|A_1|,\dots, N_n = |A_n|$ the corresponding cardinalities. Let $k= |v(\mathbf{a})|$, where $v(\mathbf{a})$ is the multiplicity function and $N$ the number of support points, with $N=N_1 \cdot \ldots \cdot N_n$. The computational complexity of $H_{\left( i,a\right) }\left( x_{i}\right)$ in (\ref{Hmikra}), for all $i\in \left\{ 1,\dots,n\right\} $ and $a\in A_{i}$, is
\begin{equation}\label{comp1}
   ((N_1-1)+\dots+(N_n-1))\cdot c_1=(N_1+\dots+N_n -n)k c_1,
\end{equation}
where $c_1$ is a constant factor.

The computational complexity of $H_{(\mathbf{a},\mathbf{k})}$ in (\ref{Hmegala}), for every $\mathbf{a} \in \mathbf{A}$ and $\mathbf{k} \in [\mathbf{0},v(\mathbf{a})-\mathbf{1}]$, is
\begin{equation} \label{comp2}
    N\cdot n \cdot k \cdot c_2,
\end{equation}
where $c_2$ is a constant factor.

The computational complexity introduced by the calculation of inverse of  matrices $\Lambda _{\mathbf{a}} $  in \textcolor{black}{(\ref{mainform})}, for every $\mathbf{a} \in \mathbf{A}$ is 
\begin{equation} \label{comp3}
    \left(k^3 + k \cdot n \cdot \left( k^2 - k\right)\right) \cdot N \cdot c_3,
\end{equation}
where $c_3$ is a constant factor.

The matrix multiplications done in (\ref{mainform}) have computational complexity 
\begin{equation} \label{comp4}
    N \cdot k^2 \cdot c_4,
\end{equation}
where $c_4$ is a constant factor.

Combining (\ref{comp1}), (\ref{comp2}), (\ref{comp3}), and (\ref{comp4}), the resulting complexity is 
\begin{equation}\label{compl_ours}
    \left(N_1+\dots+N_n -n\right) \cdot k \cdot c_1 + N\cdot n \cdot k \cdot c_2 +\left(k^3 + k \cdot n \cdot \left( k^2 - k\right)\right) \cdot N \cdot c_3 +N\cdot k^2\cdot c_4 = O(k^3 \cdot n \cdot N).
\end{equation}

Regarding the computational complexity resulting from the closed form expression in  \cite[Theorem 4.2]{fractmult}: The computational burden of calculating all  $ H_{a_j}(x_j)$ and $G_{a_{j}}^{k_{j}}$ is
\begin{equation*}
    (N_1+\cdots +N_n -n)\cdot k+ N\cdot k^2\cdot c_5,
\end{equation*}
and the resulting complexity in order to compute (\ref{ndpolmeh}) is 
\begin{equation}\label{compl_Pandey}
N_1+\cdots +N_n -n + N^2 \cdot k^{n+2} \cdot n \cdot c_6 = O(N^2 \cdot k^{n+2} \cdot n).
\end{equation}
where $c_5,c_6$ are  constant factors.

It becomes obvious that the computational complexity of the \textcolor{black}{Hermite interpolant} in the form of \cite[Theorem 4.2]{fractmult} is not polynomial with respect to $k$, whereas the complexity of the proposed Hermite interpolant is of polynomial time with respect to $k$. }
%It is also worth mentioning that the polynomials $G^{k}_{a}$ in (\ref{polspy}) have maximum degree $\nu_{i}(a) \cdot (n-1) + \nu_{i}(a) -k -1 +$, whereas the maximum degree is $\nu_{i}(a) \cdot (n-1) + \nu_{i}(a) -k -1$
\end{rem}
